Delaunay stability via perturbations

We present an algorithm that takes as input a finite point set in Euclidean space, and performs a perturbation that guarantees that the Delaunay triangulation of the resulting perturbed point set has quantifiable stability with respect to the metric and the point positions. There is also a guarantee on the quality of the simplices: they cannot be too flat. The algorithm provides an alternative tool to the weighting or refinement methods to remove poorly shaped simplices in Delaunay triangulations of arbitrary dimension, but in addition it provides a guarantee of stability for the resulting triangulation.

==> Makefile <==
#
# Makefile for flat perturbation algorithm
# 20120921
#

TEXINPUTS := .:./styles//:
	export TEXINPUTS

papers=ijcga_flatpert flat_pert inria_flatpert cgl_flatpert #esa_short


default: flat_pert.bbl

plain: flat_pert.bbl

ijcga: ijcga_flatpert.bbl

cgl: cgl_flatpert.bbl

inria: inria_flatpert.bbl

all: $(addsuffix .pdf,$(basename ${papers}))

bib: $(addsuffix .bbl,$(basename ${papers}))

%.pdf: %.tex *.tex
	pdflatex $<
	pdflatex $<

%.bbl: %.pdf *.bib
	bibtex $(basename $<)
	pdflatex $(basename $<)
	pdflatex $(basename $<)

clean:
	rm -f *.bbl *.blg *.aux *.out *.log *.brf *.thm *.toc \
$(addsuffix .pdf,$(basename ${papers}))

cleanmax: clean
	rm -f *~ lablst.pdf



==> precision.tex <==
% -*- LaTeX -*-
% precision.tex
% 20121129
% 

\newcommand{\errpred}{e_{\alpha}}
\newcommand{\errinsphere}{e_S}
\newcommand{\highhoop}{\alpha_H}
\newcommand{\lowhoop}{\alpha_L}
\newcommand{\highflake}{\Gamma_H}

\section{Precision requirements}
\label{sec:precision}

We can estimate the order of magnitude of the precision requirements
associated with the algorithm by considering error tolerances without
specifically analysing the computation of the geometric predicate.

\Algref{alg1} needs to evaluate the geometric predicate
\begin{equation}
  \label{eq:the.predicate}
  \abs{\distEm{x}{\circcentre{\splxs}} - \circrad{\splxs}} - \hoopbnd
  2\samconst \leq 0
\end{equation}
that appears in \Algref{alg:good.perturbation}. This is essentially an
``insphere'' predicate, but the sphere $\diasphere{\splxs}$ may be
defined by a simplex $\splxs$ whose dimension is less than $m$.  If we
are to guarantee that the algorithm will terminate with given desired
effective values of $\delta_0$ and $\flakebnd$, there is an upper
bound on the error that can be tolerated in the evaluation of
Predicate~\eqref{eq:the.predicate}. The magnitude of this error gives
us an estimate of the precision required to run the algorithm with
these parameters; the actual value of the required precision depends
on the details of how Predicate~\eqref{eq:the.predicate} is evaluated.

For simplicity we set $\sparseconst = 1$ and $\samconst = 1$. Let
$\errpred$ be the error incurred in the evaluation of
Predicate~\eqref{eq:the.predicate}. This error can be bounded because
Properties \ref{hyp:good.facets} and
\ref{hyp:clean.facet.rad.bnd} of \Thmref{thm:prop.forbid.cfg} ensure
that Predicate~\eqref{eq:the.predicate} does not need to be evaluated
on arbitrarily thin simplices.

We consider $\hoopbnd$ to be a parameter that we give to the
algorithm. Then in order to exploit our termination guarantees, we
need to consider the largest possible hoop parameter that could be
implicit in a computation. In other words, the hoop parameter
determines the volume of the bad perturbations within the perturbation
ball, see \Figref{fig:forbidden.volume}, and if the error in the
evaluation of Predicate~\eqref{eq:the.predicate} is too large we lose
the guarantee that a good perturbation will be found. We say the error
induces an implicit hoop parameter which we express as $\highhoop$,
where
\begin{equation*}
  2\highhoop = 2\hoopbnd + \errpred.
\end{equation*}
Using Property~\ref{hyp:clean.hoop.bnd} of
\Thmref{thm:prop.forbid.cfg}, we write $\highhoop = 2^{13}
\highflake$, where $\highflake$ is \emph{defined} by this equation,
and represents the largest flake parameter that could be implicit in a
calculation. For the goals of the current argument, we may assume that
$m \leq 5$, so that $\ballvol{m-1}/\ballvolm < 1$, and we can ignore
this factor in the definition of $K$ that appears in
\Eqnref{eq:raw.K}.  Then, letting $\pertbnd = 2^{-2}$,
\Eqnref{eq:raw.gamma.z.bnd} demands
\begin{equation*}
  \hoopbnd + \frac{\errpred}{2} = 2^{13} \highflake < 2^{11} K^{-1} =
  2^{-(3m^2 + 4m + 5)} \stackrel{\text{def}}{=} Z. 
\end{equation*}
We observe that in order to guarantee termination of the algorithm we
require $\errpred < 2Z$. Similarly, we must choose $\hoopbnd$ to be
less than $Z$. It is convenient to write $\hoopbnd = 2^{-j}Z$ and
$\errpred = 2^{-(k-1)}Z$ for positive integers $j$ and $k$. In order
to estimate the effective $\delta_0$ and $\flakebnd$ that we can hope
to attain, we choose $j=1$. We then observe, again from
Property~\ref{hyp:clean.hoop.bnd}, that the flake parameter that we
can actually guarantee is given by $\flakebnd = 2^{-13}\lowhoop$,
where
\begin{equation*}
  \lowhoop  = \hoopbnd - \frac{\errpred}{2} = (2^{-1} - 2^{-k})Z.
\end{equation*}
Assuming $k \geq 2$, we have $\flakebnd \geq 2^{-15}Z$. 

We can now give estimates for the largest magnitudes of the parameters
$\delta_0 = \flakebnd^{m+1}$ that we could hope to attain. If $m=2$,
then $Z = 2^{-25}$ and we need $\errpred \leq 2^{-26}$ in order to
obtain $\flakebnd = 2^{-40}$ and $\delta_0 = 2^{-120}$. If $m=3$, then
$\errpred \leq 2^{-45}$ yields $\flakebnd = 2^{-59}$ and $\delta_0 =
2^{-236}$. These small values for $\delta_0$ do not indicate a
practical relevance for the perturbation algorithm.
% an indication that the
% pertubation algorithm in its current form does not provide a level of
% genericity that will be of practical value in any dimension. 
However, the algorithm is formulated for arbitrary dimensions, and in
dimension 2 in particular, it does not make sense to consider flakes
and a parameter $\flakebnd$. Indeed, in two dimensions the altitudes
of the facets of our \hoop s will be already bounded by the sampling
parameters $\sparseconst$ and $\samconst$.

Given a \pueset\ $\ppts$, that is $\delta$-generic, the restricted
Delaunay triangulation $\rdelppts$ around points sufficently far from
the boundary of $\convhull{\ppts}$ can in principle be computed using
floating point arithmetic. We estimate the order of magnitude of the
precision required to evaluate the \texttt{insphere}$(x,\splxs^m)$
predicate, assuming that $\ppts$ is the output of \Algref{alg1} with
guaranteed $\delta_0$ and $\flakebnd$ as discussed above. We can write
the insphere predicate as~\cite{funke2005}
\begin{equation}
  \label{eq:insphere.orient}
  \text{\texttt{insphere}}(x,\splxs^m) =
  \text{\texttt{orient}}(\splxs^m)(\distEm{x}{\circcentre{\splxs^m}}^2 -
  \circrad{\splxs^m}^2), 
\end{equation}
where \texttt{insphere} and \texttt{orient} represent determinants
\cite{funke2005}. The \texttt{insphere} predicate is what needs to be
evaluated to compute the Delaunay triangulation; we will use the right
hand side of inequality~\eqref{eq:insphere.orient} to estimate the
magnitude of the error that can be tolerated while still guaranteeing
that \texttt{insphere} produces the correct sign.

Again assuming $\sparseconst = 1$ and $\samconst = 1$, we have
$\psparseconst \psamconst = \frac{1}{2}$ and putting $R =
\distEm{x}{\circcentre{\splxs^m}}$ we get
\begin{equation*}
  \abs{R^2 - \circrad{\splxs^m}^2} \geq \circrad{\splxs^m} \abs{R -
    \circrad{\splxs^m}} \geq \frac{\psparseconst \psamconst}{2}
  \delta_0\psparseconst \psamconst = 2^{-3} \delta_0. 
\end{equation*}

The \texttt{orient} predicate represents $m!$ times the signed volume
of $\splxs^m$.  The absolute value of this can be expressed as a
telescopic product of altitudes of faces of progressively lower
dimension.  If $\splxs^m$ is not $\flakebnd$-good, then it cannot be a
Delaunay simplex. This could be tested by evaluating the magnitude of
\texttt{orient} for example. We assume then that $\splxs^m$ is
$\flakebnd$-good. Then the altitude of a $j$-dimensional face
$\splxs^j \leq \splxs^m$ is bounded below by $j
\thickness{\splxs^j}\longedge{\splxs} \geq \frac{1}{2} j \flakebnd^j
$. It follows then that
\begin{equation*}
  \abs{ \text{\texttt{orient}}(\splxs^m) } \geq 2^{-m}
  \flakebnd^{\frac{m(m+1)}{2}}. 
\end{equation*}

Let $\errinsphere$ be the error incurred in the evaluation of
\texttt{insphere}.  The preceding observations, together with
\Eqnref{eq:insphere.orient}, imply that \texttt{insphere} will
evaluate to the correct sign provided that
\begin{equation*}
  \errinsphere  < 2^{-(m+3)} \flakebnd^{\frac{m(m+1)}{2}} \delta_0
  \leq 2^{-(m+3)} \flakebnd^{\frac{1}{2}m^2 + \frac{3}{2}m + 1}.
\end{equation*}
% For $m = 2$ we found we could obtain $\flakebnd = 2^{-40}$, and this
% implies that we would require $\errinsphere < 2^{-245}$. Thus although
% our algorithm in principle provides the ingredients for a controlled
% perturbation scheme, the practical relevance to robust computation is
% not evident from the current analysis.
Using the bound $\flakebnd = 2^{-15}Z$ found above, we find that we
require $\errinsphere < 2^{\bigo{m^4}}$.
% , and the exponent could be written explicitly as $\frac{3}{2}m^4 +
% \frac{13}{2}m^3 + 19m^2 + 35m + 23$.




